Machine Learning based Extraction of Boundary Conditions from Doppler Echo Images for Patient Specific Coarctation of the Aorta: Computational Fluid Dynamics Study

Purpose- Coarctation of the Aorta (CoA) patient-specific computational fluid dynamics (CFD) studies in resource constrained settings are limited by the available imaging modalities for geometry and velocity data acquisition. Doppler echocardiography has been seen as a suitable velocity acquisition modality due to its higher availability and safety. This study aimed to investigate the application of classical machine learning (ML) methods to create an adequate and robust approach for obtaining boundary conditions (BCs) from Doppler Echocardiography images, for haemodynamic modeling using CFD. Methods- Our proposed approach combines ML and CFD to model haemodynamic flow within the region of interest. With the key feature of the approach being the use of ML models to calibrate the inlet and outlet boundary conditions (BCs) of the CFD model. The key input variable for the ML model was the patients heart rate as this was the parameter that varied in time across the measured vessels within the study. ANSYS Fluent was used for the CFD component of the study whilst the scikit-learn python library was used for the ML component. Results- We validated our approach against a real clinical case of severe CoA before intervention. The maximum coarctation velocity of our simulations were compared to the measured maximum coarctation velocity obtained from the patient whose geometry is used within the study. Of the 5 ML models used to obtain BCs the top model was within 5\% of the measured maximum coarctation velocity. Conclusion- The framework demonstrated that it was capable of taking variations of the patients heart rate between measurements into account. Thus, enabling the calculation of BCs that were physiologically realistic when the heart rate was scaled across each vessel whilst providing a reasonably accurate solution.

==> references.tex <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{27}
% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\url{https://doi.org/#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\bibcommenthead
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

%%% 1
\bibitem{Liu2019CHD}
\begin{barticle}
\bauthor{\bsnm{Liu}, \binits{Y.}},
\bauthor{\bsnm{Chen}, \binits{S.}},
\bauthor{\bsnm{Zühlke}, \binits{L.}},
\bauthor{\bsnm{Black}, \binits{G.C.}},
\bauthor{\bsnm{Choy}, \binits{M.-k.}},
\bauthor{\bsnm{Li}, \binits{N.}},
\bauthor{\bsnm{Keavney}, \binits{B.D.}}:
\batitle{{Global birth prevalence of congenital heart defects 1970–2017:
  updated systematic review and meta-analysis of 260 studies}}.
\bjtitle{International Journal of Epidemiology}
\bvolume{48}(\bissue{2}),
\bfpage{455}--\blpage{463}
(\byear{2019})
{\href{https://arxiv.org/abs/https://academic.oup.com/ije/article-pdf/48/2/455/28479664/dyz009.pdf}{{https://academic.oup.com/ije/article-pdf/48/2/455/28479664/dyz009.pdf}}}.
\doiurl{10.1093/ije/dyz009}
\end{barticle}
\endbibitem

%%% 2
\bibitem{zuhlke2019congenital}
\begin{barticle}
\bauthor{\bsnm{Z{\"u}hlke}, \binits{L.}},
\bauthor{\bsnm{Lawrenson}, \binits{J.}},
\bauthor{\bsnm{Comitis}, \binits{G.}},
\bauthor{\bsnm{De~Decker}, \binits{R.}},
\bauthor{\bsnm{Brooks}, \binits{A.}},
\bauthor{\bsnm{Fourie}, \binits{B.}},
\bauthor{\bsnm{Swanson}, \binits{L.}},
\bauthor{\bsnm{Hugo-Hamman}, \binits{C.}}:
\batitle{Congenital heart disease in low-and lower-middle--income countries:
  current status and new opportunities}.
\bjtitle{Current cardiology reports}
\bvolume{21}(\bissue{12}),
\bfpage{1}--\blpage{13}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 3
\bibitem{obaid2019computer}
\begin{barticle}
\bauthor{\bsnm{Obaid}, \binits{D.R.}},
\bauthor{\bsnm{Smith}, \binits{D.}},
\bauthor{\bsnm{Gilbert}, \binits{M.}},
\bauthor{\bsnm{Ashraf}, \binits{S.}},
\bauthor{\bsnm{Chase}, \binits{A.}}:
\batitle{Computer simulated “virtual tavr” to guide tavr in the presence of
  a previous starr-edwards mitral prosthesis}.
\bjtitle{Journal of Cardiovascular Computed Tomography}
\bvolume{13}(\bissue{1}),
\bfpage{38}--\blpage{40}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 4
\bibitem{cecchi2011recoarctation}
\begin{barticle}
\bauthor{\bsnm{Cecchi}, \binits{E.}},
\bauthor{\bsnm{Giglioli}, \binits{C.}},
\bauthor{\bsnm{Valente}, \binits{S.}},
\bauthor{\bsnm{Lazzeri}, \binits{C.}},
\bauthor{\bsnm{Gensini}, \binits{G.F.}},
\bauthor{\bsnm{Abbate}, \binits{R.}},
\bauthor{\bsnm{Mannini}, \binits{L.}}:
\batitle{Role of hemodynamic shear stress in cardiovascular disease}.
\bjtitle{Atherosclerosis}
\bvolume{214}(\bissue{2}),
\bfpage{249}--\blpage{256}
(\byear{2011}).
\doiurl{10.1016/j.atherosclerosis.2010.09.008}
\end{barticle}
\endbibitem

%%% 5
\bibitem{swanson2020patient}
\begin{barticle}
\bauthor{\bsnm{Swanson}, \binits{L.}},
\bauthor{\bsnm{Owen}, \binits{B.}},
\bauthor{\bsnm{Keshmiri}, \binits{A.}},
\bauthor{\bsnm{Deyranlou}, \binits{A.}},
\bauthor{\bsnm{Aldersley}, \binits{T.}},
\bauthor{\bsnm{Lawrenson}, \binits{J.}},
\bauthor{\bsnm{Human}, \binits{P.}},
\bauthor{\bsnm{De~Decker}, \binits{R.}},
\bauthor{\bsnm{Fourie}, \binits{B.}},
\bauthor{\bsnm{Comitis}, \binits{G.}}, \betal:
\batitle{A patient-specific cfd pipeline using doppler echocardiography for
  application in coarctation of the aorta in a limited resource clinical
  context}.
\bjtitle{Frontiers in Bioengineering and Biotechnology}
\bvolume{8},
\bfpage{409}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 6
\bibitem{capelli2018patient}
\begin{barticle}
\bauthor{\bsnm{Capelli}, \binits{C.}},
\bauthor{\bsnm{Sauvage}, \binits{E.}},
\bauthor{\bsnm{Giusti}, \binits{G.}},
\bauthor{\bsnm{Bosi}, \binits{G.M.}},
\bauthor{\bsnm{Ntsinjana}, \binits{H.}},
\bauthor{\bsnm{Carminati}, \binits{M.}},
\bauthor{\bsnm{Derrick}, \binits{G.}},
\bauthor{\bsnm{Marek}, \binits{J.}},
\bauthor{\bsnm{Khambadkone}, \binits{S.}},
\bauthor{\bsnm{Taylor}, \binits{A.M.}}, \betal:
\batitle{Patient-specific simulations for planning treatment in congenital
  heart disease}.
\bjtitle{Interface Focus}
\bvolume{8}(\bissue{1}),
\bfpage{20170021}
(\byear{2018})
\end{barticle}
\endbibitem

%%% 7
\bibitem{pc_mri_1}
\begin{barticle}
\bauthor{\bsnm{Pirola}, \binits{S.}},
\bauthor{\bsnm{Jarral}, \binits{O.}},
\bauthor{\bsnm{O'Regan}, \binits{D.}},
\bauthor{\bsnm{Asimakopoulos}, \binits{G.}},
\bauthor{\bsnm{Anderson}, \binits{J.}},
\bauthor{\bsnm{Pepper}, \binits{J.}},
\bauthor{\bsnm{Athanasiou}, \binits{T.}},
\bauthor{\bsnm{Xu}, \binits{X.}}:
\batitle{Computational study of aortic hemodynamics for patients with an
  abnormal aortic valve: The importance of secondary flow at the ascending
  aorta inlet}.
\bjtitle{APL bioengineering}
\bvolume{2}(\bissue{2}),
\bfpage{026101}
(\byear{2018})
\end{barticle}
\endbibitem

%%% 8
\bibitem{pc_mri_2}
\begin{barticle}
\bauthor{\bsnm{Antonuccio}, \binits{M.N.}},
\bauthor{\bsnm{Mariotti}, \binits{A.}},
\bauthor{\bsnm{Fanni}, \binits{B.M.}},
\bauthor{\bsnm{Capellini}, \binits{K.}},
\bauthor{\bsnm{Capelli}, \binits{C.}},
\bauthor{\bsnm{Sauvage}, \binits{E.}},
\bauthor{\bsnm{Celi}, \binits{S.}}:
\batitle{Effects of uncertainty of outlet boundary conditions in a
  patient-specific case of aortic coarctation}.
\bjtitle{Annals of biomedical engineering}
\bvolume{49}(\bissue{12}),
\bfpage{3494}--\blpage{3507}
(\byear{2021})
\end{barticle}
\endbibitem

%%% 9
\bibitem{pc_mri_3}
\begin{barticle}
\bauthor{\bsnm{Br{\"u}ning}, \binits{J.}},
\bauthor{\bsnm{Hellmeier}, \binits{F.}},
\bauthor{\bsnm{Yevtushenko}, \binits{P.}},
\bauthor{\bsnm{K{\"u}hne}, \binits{T.}},
\bauthor{\bsnm{Goubergrits}, \binits{L.}}:
\batitle{Uncertainty quantification for non-invasive assessment of pressure
  drop across a coarctation of the aorta using cfd}.
\bjtitle{Cardiovascular engineering and technology}
\bvolume{9}(\bissue{4}),
\bfpage{582}--\blpage{596}
(\byear{2018})
\end{barticle}
\endbibitem

%%% 10
\bibitem{pc_mri_4}
\begin{botherref}
\oauthor{\bsnm{Campbell}, \binits{I.C.}},
\oauthor{\bsnm{Ries}, \binits{J.}},
\oauthor{\bsnm{Dhawan}, \binits{S.S.}},
\oauthor{\bsnm{Quyyumi}, \binits{A.A.}},
\oauthor{\bsnm{Taylor}, \binits{W.R.}},
\oauthor{\bsnm{Oshinski}, \binits{J.N.}}:
Effect of inlet velocity profiles on patient-specific computational fluid
  dynamics simulations of the carotid bifurcation.
Journal of biomechanical engineering
\textbf{134}(5)
(2012)
\end{botherref}
\endbibitem

%%% 11
\bibitem{pc_mri_5}
\begin{barticle}
\bauthor{\bsnm{Conti}, \binits{M.}},
\bauthor{\bsnm{Long}, \binits{C.}},
\bauthor{\bsnm{Marconi}, \binits{M.}},
\bauthor{\bsnm{Berchiolli}, \binits{R.}},
\bauthor{\bsnm{Bazilevs}, \binits{Y.}},
\bauthor{\bsnm{Reali}, \binits{A.}}:
\batitle{Carotid artery hemodynamics before and after stenting: A patient
  specific cfd study}.
\bjtitle{Computers \& Fluids}
\bvolume{141},
\bfpage{62}--\blpage{74}
(\byear{2016})
\end{barticle}
\endbibitem

%%% 12
\bibitem{bishop2016pattern}
\begin{bbook}
\bauthor{\bsnm{Bishop}, \binits{C.M.}}:
\bbtitle{Pattern Recognition and Machine Learning}.
\bsertitle{Information Science and Statistics}.
\bpublisher{Springer}, \blocation{???}
(\byear{2016}).
\burl{https://books.google.co.za/books?id=kOXDtAEACAAJ}
\end{bbook}
\endbibitem

%%% 13
\bibitem{feiger2020accelerating}
\begin{barticle}
\bauthor{\bsnm{Feiger}, \binits{B.}},
\bauthor{\bsnm{Gounley}, \binits{J.}},
\bauthor{\bsnm{Adler}, \binits{D.}},
\bauthor{\bsnm{Leopold}, \binits{J.A.}},
\bauthor{\bsnm{Draeger}, \binits{E.W.}},
\bauthor{\bsnm{Chaudhury}, \binits{R.}},
\bauthor{\bsnm{Ryan}, \binits{J.}},
\bauthor{\bsnm{Pathangey}, \binits{G.}},
\bauthor{\bsnm{Winarta}, \binits{K.}},
\bauthor{\bsnm{Frakes}, \binits{D.}}, \betal:
\batitle{Accelerating massively parallel hemodynamic models of coarctation of
  the aorta using neural networks}.
\bjtitle{Scientific reports}
\bvolume{10}(\bissue{1}),
\bfpage{1}--\blpage{13}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 14
\bibitem{nita2022personalized}
\begin{barticle}
\bauthor{\bsnm{Nita}, \binits{C.-I.}},
\bauthor{\bsnm{Puiu}, \binits{A.}},
\bauthor{\bsnm{Bunescu}, \binits{D.}},
\bauthor{\bsnm{Mihai~Itu}, \binits{L.}},
\bauthor{\bsnm{Mihalef}, \binits{V.}},
\bauthor{\bsnm{Chintalapani}, \binits{G.}},
\bauthor{\bsnm{Armstrong}, \binits{A.}},
\bauthor{\bsnm{Zampi}, \binits{J.}},
\bauthor{\bsnm{Benson}, \binits{L.}},
\bauthor{\bsnm{Sharma}, \binits{P.}}, \betal:
\batitle{Personalized pre-and post-operative hemodynamic assessment of aortic
  coarctation from 3d rotational angiography}.
\bjtitle{Cardiovascular Engineering and Technology}
\bvolume{13}(\bissue{1}),
\bfpage{14}--\blpage{40}
(\byear{2022})
\end{barticle}
\endbibitem

%%% 15
\bibitem{yevtushenko2021deep}
\begin{botherref}
\oauthor{\bsnm{Yevtushenko}, \binits{P.}},
\oauthor{\bsnm{Goubergrits}, \binits{L.}},
\oauthor{\bsnm{Gundelwein}, \binits{L.}},
\oauthor{\bsnm{Setio}, \binits{A.}},
\oauthor{\bsnm{Heimann}, \binits{T.}},
\oauthor{\bsnm{Ramm}, \binits{H.}},
\oauthor{\bsnm{Lamecker}, \binits{H.}},
\oauthor{\bsnm{Kuehne}, \binits{T.}},
\oauthor{\bsnm{Meyer}, \binits{A.}},
\oauthor{\bsnm{Schafstedde}, \binits{M.}}:
Deep learning based centerline-aggregated aortic hemodynamics: An efficient
  alternative to numerical modelling of hemodynamics.
IEEE Journal of Biomedical and Health Informatics
(2021)
\end{botherref}
\endbibitem

%%% 16
\bibitem{raissi2019pinn}
\begin{barticle}
\bauthor{\bsnm{Raissi}, \binits{M.}},
\bauthor{\bsnm{Perdikaris}, \binits{P.}},
\bauthor{\bsnm{Karniadakis}, \binits{G.E.}}:
\batitle{Physics-informed neural networks: A deep learning framework for
  solving forward and inverse problems involving nonlinear partial differential
  equations}.
\bjtitle{Journal of Computational Physics}
\bvolume{378},
\bfpage{686}--\blpage{707}
(\byear{2019}).
\doiurl{10.1016/j.jcp.2018.10.045}
\end{barticle}
\endbibitem

%%% 17
\bibitem{madhavan2018effect}
\begin{barticle}
\bauthor{\bsnm{Madhavan}, \binits{S.}},
\bauthor{\bsnm{Kemmerling}, \binits{E.M.C.}}:
\batitle{The effect of inlet and outlet boundary conditions in image-based cfd
  modeling of aortic flow}.
\bjtitle{Biomedical engineering online}
\bvolume{17}(\bissue{1}),
\bfpage{1}--\blpage{20}
(\byear{2018})
\end{barticle}
\endbibitem

%%% 18
\bibitem{morbiducci2013inflow}
\begin{barticle}
\bauthor{\bsnm{Morbiducci}, \binits{U.}},
\bauthor{\bsnm{Ponzini}, \binits{R.}},
\bauthor{\bsnm{Gallo}, \binits{D.}},
\bauthor{\bsnm{Bignardi}, \binits{C.}},
\bauthor{\bsnm{Rizzo}, \binits{G.}}:
\batitle{Inflow boundary conditions for image-based computational hemodynamics:
  impact of idealized versus measured velocity profiles in the human aorta}.
\bjtitle{Journal of biomechanics}
\bvolume{46}(\bissue{1}),
\bfpage{102}--\blpage{109}
(\byear{2013})
\end{barticle}
\endbibitem

%%% 19
\bibitem{pirola2017choice}
\begin{barticle}
\bauthor{\bsnm{Pirola}, \binits{S.}},
\bauthor{\bsnm{Cheng}, \binits{Z.}},
\bauthor{\bsnm{Jarral}, \binits{O.}},
\bauthor{\bsnm{O'Regan}, \binits{D.}},
\bauthor{\bsnm{Pepper}, \binits{J.}},
\bauthor{\bsnm{Athanasiou}, \binits{T.}},
\bauthor{\bsnm{Xu}, \binits{X.}}:
\batitle{On the choice of outlet boundary conditions for patient-specific
  analysis of aortic flow using computational fluid dynamics}.
\bjtitle{Journal of biomechanics}
\bvolume{60},
\bfpage{15}--\blpage{21}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 20
\bibitem{hands-on}
\begin{bbook}
\bauthor{\bsnm{G\`{e}ron}, \binits{A.}}:
\bbtitle{Hands-on Machine Learning with Scikit-Learn and TensorFlow : Concepts,
  Tools, and Techniques to Build Intelligent Systems}.
\bpublisher{O'Reilly Media},
\blocation{Sebastopol, CA}
(\byear{2017})
\end{bbook}
\endbibitem

%%% 21
\bibitem{plotdigitizer}
\begin{botherref}
PlotDigitizer: Version 2.2
(2022).
\url{https://plotdigitizer.com}
\end{botherref}
\endbibitem

%%% 22
\bibitem{sklearn}
\begin{barticle}
\bauthor{\bsnm{Pedregosa}, \binits{F.}},
\bauthor{\bsnm{Varoquaux}, \binits{G.}},
\bauthor{\bsnm{Gramfort}, \binits{A.}},
\bauthor{\bsnm{Michel}, \binits{V.}},
\bauthor{\bsnm{Thirion}, \binits{B.}},
\bauthor{\bsnm{Grisel}, \binits{O.}},
\bauthor{\bsnm{Blondel}, \binits{M.}},
\bauthor{\bsnm{Prettenhofer}, \binits{P.}},
\bauthor{\bsnm{Weiss}, \binits{R.}},
\bauthor{\bsnm{Dubourg}, \binits{V.}}, \betal:
\batitle{Scikit-learn: Machine learning in python}.
\bjtitle{Journal of machine learning research}
\bvolume{12}(\bissue{Oct}),
\bfpage{2825}--\blpage{2830}
(\byear{2011})
\end{barticle}
\endbibitem

%%% 23
\bibitem{numpy}
\begin{barticle}
\bauthor{\bsnm{Harris}, \binits{C.R.}},
\bauthor{\bsnm{Millman}, \binits{K.J.}},
\bauthor{\bparticle{van~der} \bsnm{Walt}, \binits{S.J.}},
\bauthor{\bsnm{Gommers}, \binits{R.}},
\bauthor{\bsnm{Virtanen}, \binits{P.}},
\bauthor{\bsnm{Cournapeau}, \binits{D.}},
\bauthor{\bsnm{Wieser}, \binits{E.}},
\bauthor{\bsnm{Taylor}, \binits{J.}},
\bauthor{\bsnm{Berg}, \binits{S.}},
\bauthor{\bsnm{Smith}, \binits{N.J.}},
\bauthor{\bsnm{Kern}, \binits{R.}},
\bauthor{\bsnm{Picus}, \binits{M.}},
\bauthor{\bsnm{Hoyer}, \binits{S.}},
\bauthor{\bparticle{van} \bsnm{Kerkwijk}, \binits{M.H.}},
\bauthor{\bsnm{Brett}, \binits{M.}},
\bauthor{\bsnm{Haldane}, \binits{A.}},
\bauthor{\bparticle{Fernández~del} \bsnm{Río}, \binits{J.}},
\bauthor{\bsnm{Wiebe}, \binits{M.}},
\bauthor{\bsnm{Peterson}, \binits{P.}},
\bauthor{\bsnm{Gérard-Marchant}, \binits{P.}},
\bauthor{\bsnm{Sheppard}, \binits{K.}},
\bauthor{\bsnm{Reddy}, \binits{T.}},
\bauthor{\bsnm{Weckesser}, \binits{W.}},
\bauthor{\bsnm{Abbasi}, \binits{H.}},
\bauthor{\bsnm{Gohlke}, \binits{C.}},
\bauthor{\bsnm{Oliphant}, \binits{T.E.}}:
\batitle{Array programming with {NumPy}}.
\bjtitle{Nature}
\bvolume{585},
\bfpage{357}--\blpage{362}
(\byear{2020}).
\doiurl{10.1038/s41586-020-2649-2}
\end{barticle}
\endbibitem

%%% 24
\bibitem{ke2017lightgbm}
\begin{botherref}
\oauthor{\bsnm{Ke}, \binits{G.}},
\oauthor{\bsnm{Meng}, \binits{Q.}},
\oauthor{\bsnm{Finley}, \binits{T.}},
\oauthor{\bsnm{Wang}, \binits{T.}},
\oauthor{\bsnm{Chen}, \binits{W.}},
\oauthor{\bsnm{Ma}, \binits{W.}},
\oauthor{\bsnm{Ye}, \binits{Q.}},
\oauthor{\bsnm{Liu}, \binits{T.-Y.}}:
Lightgbm: A highly efficient gradient boosting decision tree.
Advances in neural information processing systems
\textbf{30}
(2017)
\end{botherref}
\endbibitem

%%% 25
\bibitem{pant2014methodological}
\begin{barticle}
\bauthor{\bsnm{Pant}, \binits{S.}},
\bauthor{\bsnm{Fabr{\`e}ges}, \binits{B.}},
\bauthor{\bsnm{Gerbeau}, \binits{J.-F.}},
\bauthor{\bsnm{Vignon-Clementel}, \binits{I.}}:
\batitle{A methodological paradigm for patient-specific multi-scale cfd
  simulations: from clinical measurements to parameter estimates for individual
  analysis}.
\bjtitle{International journal for numerical methods in biomedical engineering}
\bvolume{30}(\bissue{12}),
\bfpage{1614}--\blpage{1648}
(\byear{2014})
\end{barticle}
\endbibitem

%%% 26
\bibitem{lassila2020population}
\begin{barticle}
\bauthor{\bsnm{Lassila}, \binits{T.}},
\bauthor{\bsnm{Sarrami-Foroushani}, \binits{A.}},
\bauthor{\bsnm{Hejazi}, \binits{S.}},
\bauthor{\bsnm{Frangi}, \binits{A.F.}}:
\batitle{Population-specific modelling of between/within-subject flow
  variability in the carotid arteries of the elderly}.
\bjtitle{International Journal for Numerical Methods in Biomedical Engineering}
\bvolume{36}(\bissue{1}),
\bfpage{3271}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 27
\bibitem{rackauckas2020universal}
\begin{botherref}
\oauthor{\bsnm{Rackauckas}, \binits{C.}},
\oauthor{\bsnm{Ma}, \binits{Y.}},
\oauthor{\bsnm{Martensen}, \binits{J.}},
\oauthor{\bsnm{Warner}, \binits{C.}},
\oauthor{\bsnm{Zubov}, \binits{K.}},
\oauthor{\bsnm{Supekar}, \binits{R.}},
\oauthor{\bsnm{Skinner}, \binits{D.}},
\oauthor{\bsnm{Ramadhan}, \binits{A.}},
\oauthor{\bsnm{Edelman}, \binits{A.}}:
Universal differential equations for scientific machine learning.
arXiv preprint arXiv:2001.04385
(2020)
\end{botherref}
\endbibitem

\end{thebibliography}

